DataCLUE: A Benchmark Suite for Data-centric NLP

Data-centric AI has recently proven to be more effective and high-performance, while traditional model-centric AI delivers fewer and fewer benefits. It emphasizes improving the quality of datasets to achieve better model performance. This field has significant potential because of its great practicability and getting more and more attention. However, we have not seen significant research progress in this field, especially in NLP. We propose DataCLUE, which is the first Data-Centric benchmark applied in NLP field. We also provide three simple but effective baselines to foster research in this field (improve Macro-F1 up to 5.7% point). In addition, we conduct comprehensive experiments with human annotators and show the hardness of DataCLUE. We also try an advanced method: the forgetting informed bootstrapping label correction method. All the resources related to DataCLUE, including datasets, toolkit, leaderboard, and baselines, is available online at https://github.com/CLUEbenchmark/DataCLUE

==> tex/Background.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\textwidth]{./pictures/inconsistency_construction.pdf}
	\caption{
		The process of CI-ToD construction.}
	\label{fig:construction-step}
\end{figure*}


\begin{figure}[t]
	\centering
	\includegraphics[scale=0.5]{./pictures/Inconsistency_type.pdf}
	\caption{
		Inconsistent types in CI-ToD. Different colors denote different inconsistent types.
	}
	\label{Inconsistency type}
\end{figure}

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{./pictures/annotation.pdf}
	\caption{
		The collection interface.
	}
	\label{annotation interface}
\end{figure*}

In our paper, the consistency identification in task-oriented dialogue is formulated as a supervised multi-label classification task, which aims to judge whether the generated system response is inconsistent.
To equip the model with the ability to analyze what the inconsistent sources lead to it, we require the model not only provide the final prediction but also the fine-grained sources including dialogue history, knowledge base (KB) and user's query.
More specifically, given a task-oriented dialogue between a user ($u$) and a system ($s$), the $n$-turned dialogue snippet consists of dialogue history $H$ = $\{(u_{1}, s_{1} ), (u_{2} , s_{2} ), ... , (u_{n-1} , s_{n-1} )\}$, the corresponding knowledge base $KB$, the user query $u_{n}$ and system response $s_{n}$.
More specifically, the task can be defined as:
\begin{eqnarray}
		\mathbf{y} = f ([H, KB, u_{n}], s_{n}), 
\end{eqnarray}
where $f$ denotes the trainable model; $\mathbf{y}$ is an output three-dimension vector, indicating whether the last utterance $s_{n}$ contradicts any previously mentioned dialogue history $H$, user query $u_{n}$ or the corresponding knowledge base $KB$ .

